Towards Robust and Expressive Whole-body Human Pose and Shape Estimation

Whole-body pose and shape estimation aims to jointly predict different behaviors (e.g., pose, hand gesture, facial expression) of the entire human body from a monocular image. Existing methods often exhibit degraded performance under the complexity of in-the-wild scenarios. We argue that the accuracy and reliability of these models are significantly affected by the quality of the predicted \textit{bounding box}, e.g., the scale and alignment of body parts. The natural discrepancy between the ideal bounding box annotations and model detection results is particularly detrimental to the performance of whole-body pose and shape estimation. In this paper, we propose a novel framework to enhance the robustness of whole-body pose and shape estimation. Our framework incorporates three new modules to address the above challenges from three perspectives: \textbf{1) Localization Module} enhances the model's awareness of the subject's location and semantics within the image space. \textbf{2) Contrastive Feature Extraction Module} encourages the model to be invariant to robust augmentations by incorporating contrastive loss with dedicated positive samples. \textbf{3) Pixel Alignment Module} ensures the reprojected mesh from the predicted camera and body model parameters are accurate and pixel-aligned. We perform comprehensive experiments to demonstrate the effectiveness of our proposed framework on body, hands, face and whole-body benchmarks. Codebase is available at \url{https://github.com/robosmplx/robosmplx}.

==> Figures/contrastive_archi.tex <==
\begin{figure*}[!ht]
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/contrastive_archi.png}
    }
    \caption{\small \textbf{Pipeline for contrastive learning.}}
    \label{figure:contrastive_archi}
\end{figure*}


==> Figures/flame.tex <==
\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-15pt}
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/face_seg.png}
    }
    \caption{\small \textbf{Examples of keypoint and part segmentation supervision for Face sub-network}}
    \label{figure:flame_supervision}
\vspace{-15pt}
\end{wrapfigure}

==> Figures/jitter.tex <==
% \begin{figure}[h!]
\begin{wrapfigure}{r}{0.45\textwidth} 
\vspace{-30pt}
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_jitter.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_jitter2.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_jitter3.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/hand_jitter.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/hand_jitter2.png}
    }
    \caption{\small \textbf{Sensitivity of existing body and hand models to different alignment}}
    \label{figure:jitter}
% \end{figure}
\vspace{-30pt}
\end{wrapfigure}

==> Figures/mano.tex <==
\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-15pt}
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/mano_seg2.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/mano_seg.png}
    }
    \caption{\small \textbf{Examples of keypoint and part segmentation supervision for Hand sub-network}}
    \label{figure:mano_supervision}
\vspace{-15pt}
\end{wrapfigure}

==> Figures/module.tex <==
\begin{figure*}[h!]
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/archi_module2.png}
    }
    % \subfigure{
    % \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/smpl_seg.png}
    % }
    \caption{\small \textbf{Architecture for sub-networks.}}
    \label{figure:module_archi}
\end{figure*}


==> Figures/scale.tex <==
% \begin{figure}[h!]
\begin{wrapfigure}{l}{0.45\textwidth} 
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_scale.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_scale2.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_scale3.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/body_scale4.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/hand_scale.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/hand_scale2.png}
    }
    \caption{\small \textbf{Sensitivity of existing body and hand models to different scale}}
    \label{figure:scale}
% \end{figure}
\end{wrapfigure}





==> Figures/smpl.tex <==


\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-15pt}
    % \captionsetup[subfigure]{labelformat=empty}
    \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/smpl_seg2.png}
    }
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/smpl_seg.png}
    }
    \caption{\small \textbf{Examples of keypoint and part segmentation supervision for Body sub-network.}}
    \label{figure:smpl_supervision}
% \end{figure}
\vspace{-15pt}
\end{wrapfigure}



==> Figures/test1.tex <==
\begin{figure}[!ht]
    % \captionsetup[subfigure]{labelformat=empty}
    % \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/test1.png}
    }
    \caption{\small \textbf{Example 1 on Expose, PIXIE, Hand4Whole, OSX, Ours}}
    % \label{figure:wholebody_errors_jitter}
\end{figure}

==> Figures/test2.tex <==
\begin{figure}[!ht]
    % \captionsetup[subfigure]{labelformat=empty}
    % \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/test2.png}
    }
    \caption{\small \textbf{Example 2 on Expose, PIXIE, Hand4Whole, OSX, Ours.}}
    % \label{figure:wholebody_errors_jitter}
\end{figure}

==> Figures/wb_errors.tex <==
\begin{figure}[!ht]
    % \captionsetup[subfigure]{labelformat=empty}
    % \centering
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/wb_errors_jitter.png}
    }
    \newpage
    \subfigure{
    \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/wb_errors_scale.png}
    }
    \caption{\small \textbf{Wholebody errors under different amounts of jitter and scale.}}
    \label{figure:wholebody_errors_jitter}
\end{figure}


% \begin{wrapfigure}{r}{0.6\textwidth} 
% \vspace{-15pt}
%     % \captionsetup[subfigure]{labelformat=empty}
%     \centering
%     \subfigure{
%     \includegraphics[width=0.9\linewidth ,keepaspectratio]{Figures/Image/wb_errors_jitter.png}
%     }
%     \caption{\small \textbf{Wholebody errors under different amounts of jitter.}}
%     \label{figure:wholebody_errors_jitter}
% \vspace{-15pt}
% \end{wrapfigure}

==> Figures_Rebuttal/iou_calculation.tex <==
\begin{wrapfigure}{r}{0.44\textwidth} 
    \centering
    \subfigure{
    \includegraphics[width=0.23\linewidth,keepaspectratio]{Figures_Rebuttal/Image/iou_calculation.png}
    }
    \caption{\small \textbf{Calculation for the Face, LHand and RHand IoU scores. The ground-truth and predicted part bounding boxes are denoted in green and red respectively.}}
    \label{figure:vis}
\end{wrapfigure}



==> Figures_Rebuttal/pixel_alignment_quantitative.tex <==
\begin{wrapfigure}{r}{0.44\textwidth} 
% \vspace{-20pt}
    \centering
    \subfigure{
    \includegraphics[width=0.23\linewidth,keepaspectratio]{Figures_Rebuttal/Image/pixel_alignment_quantitative.png}
    }
    \caption{\small \textbf{We measure the distance between projected ground-truth and predicted vertices in image space denoted in red and blue respectively to obtain Projected Vertex Errors.}}
    \label{figure:vis}
% \vspace{-15pt}
\end{wrapfigure}


==> Tables/agora.tex <==
\begin{table*}[]
% \begin{wraptable}{r}{0.42\textwidth}
\small
\centering
\caption{\small \textbf{Reconstruction errors on AGORA test set. Results obtained from evaluation platform.}}%
\vspace{-5pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c|cccc|cccc@{}}

\Xhline{1pt}
\multirow{2}{*}{\textbf{Method}}  & \multicolumn{4}{c}{\textbf{MVE}}  & \multicolumn{4}{c}{\textbf{MPJPE}}   \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \cmidrule(l){2-5} 
 & \textbf{Whole-body} &  \textbf{Body} & \textbf{Face} & \textbf{L/R Hands}  
%  \cmidrule(l){6-9} 
 & \textbf{Whole-body} & \textbf{Body} & \textbf{Face} & \textbf{L/R Hands}  \\ \Xhline{1pt}
ExPose    &  217.3  & 151.5 & 51.1 & 74.9/71.3 & 215.9 & 150.4 & 55.2 &  72.5/68.8    \\
FrankMocap    &   - & 168.3 & - & 54.7/55.7 & - & 165.2 & -  &  52.3/53.1    \\
PIXIE    &   191.8  & 142.2 & 50.2 & 49.5/49.0 & 189.3 & 140.3 & 54.5 &  46.4/46.0     \\
Hand4Whole    &   135.5  &  90.2 & 41.6 & 46.3/48.1 &  132.6 & 87.1 & 46.1 & 44.3/46.2   \\
% PyMAF-X    &  125.7 &  84.0 & 35.0 & 44.6/45.6 & 124.6 & 83.2 & 37.9  &  42.5/43.7   \\
OS-X    &  \textbf{122.8} &  \textbf{80.2} & \textbf{36.2} & 45.4/46.1& \textbf{119.9} & \textbf{78.3} & \textbf{37.9}  &  \textbf{43.0/43.9}   \\
Ours    &  132.3 &  85.0 & 39.4 & \textbf{45.3/46.1} & 129.5 & 86.4 & 39.5  &  44.5/45.2   \\
\Xhline{1pt}
\end{tabular}
\end{adjustbox}
\label{table:agora}
%\vspace{-25pt}
% \end{wraptable}
\end{table*}

==> Tables/algo_crop_scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.60\textwidth}
% \begin{table}[]
\vspace{-15pt}
\small
\caption{\small \textbf{Training and testing at different crop scales.}}%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Algorithm & Scale factor  & \multicolumn{1}{l}{PA-} & \multicolumn{1}{l}{MPJPE} & \multicolumn{1}{l}{PA-} & \multicolumn{1}{l}{PVE} \\ \midrule
HMR        & 0.2  & 9.56                         & 21.57                     & 9.26                       & 21.31                   \\
PARE & 8.73   & 0.2                      & 18.83                     & 8.52                       & 19.24                   \\ 
SPIN& 0.2 & TBC                         & TBC                      & TBC                        & TBC                    \\ 
Ours& 0.2 & TBC                          & TBC                      & TBC                        & TBC                   \\ 

\bottomrule
\label{table:algo_crop_scale_body}
\end{tabular}
% \end{table}
\end{wraptable}



==> Tables/body_jitter_scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}\textbf{}
% \begin{wraptable}{r}{0.40\textwidth}
\vspace{-5pt}
\begin{table}[H]
\small
\caption{\small \textbf{PA-MPJPE/MPJPE errors of the Body sub-network under different positional augmentations.}}%

\begin{tabular}{@{}llllllll@{}}
\toprule
       & Normal               & Transx +0.2x         & Transx -0.2x         & Transy +0.2y         & Transy -0.2y         & Scale 1.3x           & Scale 0.7x           \\ \midrule
HMR  & 67.53/112.34  & -/ - & -/-  & 86.57/ 151.15 & 77.26/148.33  & 68.46/ 117.1 & 75.38/ 124.79          \\
SPIN & 57.54/94.11  & 68.67/ 120.04 & -/ -  & 73.08/ 111.33 & 70.64/133.2  & 61.08/ 103.60 & 61.63/ 99.6          \\
PARE (HR32) & \textbf{49.35/81.79} & 77.12/ 141.71  &  -/- & 59.07/92.34  & 64.17/ 109.72 & 54.69/86.92 & \textbf{50.47/ 83.9}          \\
% Ours (DR54) & 51.02/87.07 & -/ - & -/- & \textbf{58.34/ 92.18} & \textbf{63.74/ 115.03} & \textbf{53.82/92.20} & 52.13/ 87.61 \\ \bottomrule

\label{table:body_jitter_scale}
\end{tabular}
\vspace{-15pt}
\end{table}
% \end{wraptable}

==> Tables/ehf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]

\centering
% \caption{\small \textbf{Reconstruction errors on EHF test set.}}%
\small
\caption{\small \textbf{Evaluation of wholebody network on EHF test set}}%
% \begin{tabular}{@{}lrrrrrrrrr@{}}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule

\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{l}{\textbf{PVE}}                                                              & \multicolumn{3}{l}{\textbf{PA-PVE}}                                                           & \multicolumn{3}{l}{\textbf{PA-MPJPE}}                                                    \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}\cmidrule(lr){8-10}
                        & \multicolumn{1}{l}{\textbf{Whole-body}} & \multicolumn{1}{l}{\textbf{Hands}} & \multicolumn{1}{l}{\textbf{Face}} & \multicolumn{1}{l}{\textbf{Whole-body}} & \multicolumn{1}{l}{\textbf{Body}} & \multicolumn{1}{l}{\textbf{Hands}} & \multicolumn{1}{l}{\textbf{Face}} & \multicolumn{1}{l}{\textbf{Body}} & \multicolumn{1}{l}{\textbf{Hands}} \\ 
                        \Xhline{1pt}
MTC                     & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}     & \multicolumn{1}{l}{-}    & 67.2                          & \multicolumn{1}{l}{-}    & \multicolumn{1}{l}{-}     & \multicolumn{1}{l}{-}    & 107.8                    & 16.7                      \\
SMPLify-X  \cite{Pavlakos2019}              & \multicolumn{1}{l}{-}         & \multicolumn{1}{l}{-}     & \multicolumn{1}{l}{-}    & 65.3                          & 75.4                     & 12.3                      & 6.3                      & 87.6                     & 12.9                      \\
ExPose \cite{Choutas2020}                  & 77.1                          & 51.6                      & 35                       & 54.5                          & 52.6                     & 12.8                      & 5.8                      & 62.8                     & 13.1                      \\
FrankMocap              & 107.6                         & 42.8                      & \multicolumn{1}{l}{-}    & 57.5                          & 52.7                     & 12.6                      & \multicolumn{1}{l}{-}    & 62.3                     & 12.9                      \\
PIXIE  \cite{Feng2019}                  & 89.2                          & 42.8                      & 32.7                     & 55                            & 53                       & 11.1                      & 4.6                      & 61.5                     & 11.6                      \\
Hand4Whole  \cite{Moon2022}             & 76.8                          & 39.8                      & 26.1                     & 50.3                          & \multicolumn{1}{l}{-}    & 10.8                      & 5.8                      & 60.4                     & 10.8                      \\
% PyMAF-X (Res50) \cite{Zhang2022}        & 68                            & 29.8                      & 20.5                     & 47.3                          & 45.9                     & 10.1                      & 5.6                      & 52.9                     & 10.3                      \\
% PyMAF-X (HR48)  \cite{Zhang2022}          & 64.9                          & 29.7                      & 19.7                     & 50.2                          & 44.8                     & 10.2                      & 5.5                      & 52.8                     & 10.3                      \\
OS-X (Vit-L) \cite{Lin2023}          & \textbf{70.8}                          & 53.7                      & 26.4                     & 48.7                        & -                     & 15.9                       &6.0                      & -                    & -                      \\ 
Ours (Res50)          & 73.7                          & \textbf{34.9}                      & \textbf{17.8}                     & \textbf{49.7}                         & -                     & \textbf{10.0}                       & \textbf{4.6}                      & \textbf{57.12}                     & \textbf{9.9}                      \\ 
\bottomrule
\Xhline{1pt}
\label{table:ehf}
\end{tabular}}
\vspace{-20pt}
\end{table*}

==> Tables/embedding.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.40\textwidth}
\vspace{-35pt}
% \begin{table}[]
\small
\caption{\small \textbf{Absolute difference between the top-1 retrieved pose in train set and the original pose in test set}}%
\resizebox{.4\textwidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Scale factor  & \multicolumn{1}{l}{Mean $\downarrow$} & \multicolumn{1}{l}{Std $\downarrow$} 
\\ \midrule
SimCLR         & 0.227                         & 0.0915  \\
SimCLR (+ pose-variant aug.) & 0.230                         & 0.0911     \\ 
SimCLR (+ background aug.) & 0.222                         & 0.0959     \\ 
SimCLR (+ $L_{con}$) & 0.164                         & 0.0772     \\
HMR & 0.140                         & 0.0823    \\ 
HMR (+ $L_{con}$) & 0.124                         & \textbf{0.0624}     \\
HMR (+ $L_{con}$, +ve samples)  & \textbf{0.119}                        & 0.0679     \\
\bottomrule
\label{table:embedding}
\end{tabular}}
\vspace{-25pt}
% \end{table}
\end{wraptable}




==> Tables/freihand.tex <==
\begin{wraptable}{r}{0.50\textwidth}
\vspace{-35pt}
\small
\caption{\small \textbf{Evaluation of the Hand sub-network}. $\dagger$ denotes training with extra datasets.  We report PA-MPJPE, PA-PVE and F-scores @ 5mm/10mm.}%
\resizebox{.5\textwidth}{!}{
\begin{tabular}{@{}lrrl@{}}
\toprule

\textbf{Method}                       & \multicolumn{1}{l}{PA-PVE $\downarrow$} & \multicolumn{1}{l}{PA-MPJPE $\downarrow$} & F-Scores $\uparrow$ \\ \midrule
\textbf{* Hand-only} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}           &                       \\
FreiHAND \cite{Zimmermann2019}             & 10.7                         & \multicolumn{1}{l}{-}          & 0.529/0.935           \\
Pose2Mesh \cite{Choi2020}           & 7.8                          & 7.7                            & 0.674/0.969           \\
I2L-MeshNet \cite{Moon2020}          & 7.6                          & 7.4                            & 0.681/0.973           \\
METRO (HR64) \cite{Lin2021}               & \textbf{6.7}                          & \textbf{6.8}                            & 0.717/0.981           \\
\midrule
\textbf{* Whole-body} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}           &                       \\
ExPose \cite{Pavlakos2019}              & 11.8                         & 12.2                           & 0.484/0.918           \\
Zhou et al. \cite{Zhou2021}        & -        & 15.7                           & -/-                   \\
FrankMocap \cite{Rong2021}          & 11.6                         & 9.2                            & 0.553/0.951           \\
PIXIE \cite{Feng2019}              & 12.1                         & 12                             & 0.468/0.919           \\
Hand4Whole $\dagger$ \cite{Moon2022}          & 7.7                          & 7.7                            & 0.664/0.971           \\
HMR                    & 8.6                          & 8.9                            & 0.605/0.963           \\
PyMAF  \cite{Zhang2022}                       & 8.1                          & 8.4                            & 0.638/0.969           \\
PyMAF $\dagger$ \cite{Zhang2022}                       & 7.5                          & 7.7                            & 0.671/0.974           \\ 
Ours                        &  \textbf{7.3}                          & \textbf{7.5}                            & 0.683/0.976          \\ 
Ours $\dagger$                       & \textbf{7.1}                          & \textbf{7.4}                            & 0.688/0.978          \\ 
Ours (HR64)                       & \textbf{6.7}                          & \textbf{6.9}                            & 0.715/0.981            \\ 
\bottomrule
\label{table:freihand}
\end{tabular}}
%\end{table}
\vspace{-15pt}
\end{wraptable}



==> Tables/hand_cl_augmentation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.50\textwidth}
\vspace{-15pt}
% \begin{table}[]
\small
\caption{\small \textbf{Augmentation for positive samples, using pose rotation as representation. Baseline refers to training without positive samples. FreiHand using Hand subnetwork}}%
\resizebox{.5\textwidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Augmentation  & \multicolumn{1}{l}{PA-$\downarrow$} & \multicolumn{1}{l}{MPJPE$\downarrow$} & \multicolumn{1}{l}{PA- $\downarrow$}  & \multicolumn{1}{l}{PVE$\downarrow$} 
\\ \midrule
baseline & 8.11       &      15.81            & 7.67    & 16.08 \\
color  & 7.42                         & 15.01   & 7.18 & 14.94  \\ 
pose  & 8.59      &    16.96                & 8.15    & 17.21 \\ 
location  & 7.80     & 15.98    & 7.46   & 15.56 \\   
color + location  & 7.45    & 14.94   & 7.20 & 14.77 \\ 
\bottomrule
\label{table:hand_cl_augmentation}
\end{tabular}}
\vspace{-25pt}
% \end{table}
\end{wraptable}

==> Tables/hand_cl_representation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.50\textwidth}
\vspace{-35pt}
% \begin{table}[]
\small
\caption{\small \textbf{Ablation of different representation for contrastive loss}}%
\resizebox{.5\textwidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Representation  & \multicolumn{1}{l}{PA-$\downarrow$} & \multicolumn{1}{l}{MPJPE$\downarrow$} & \multicolumn{1}{l}{PA $\downarrow$}  & \multicolumn{1}{l}{PVE$\downarrow$} 
\\ \midrule
baseline & 7.49          &15.51              & 7.46 & 15.59 \\
pose  & 8.11       &      15.81            & 7.67    & 16.08 \\ 
go + pose  & 7.71     & 14.98                    & 7.54  & 14.91  \\ 
keypoint  & 7.48          & 15.01               & 7.32   & 15.29  \\
pose, +ve  & 7.45      &    14.94                & 7.20    & 14.77 \\ 
keypoint, +ve  & 7.31                &14.62            & 7.18     & 15.01    \\   
\bottomrule
\label{table:hand_cl_representation}
\end{tabular}}
\vspace{-25pt}
% \end{table}
\end{wraptable}


==> Tables/hand_scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.60\textwidth}
% \begin{table}[]
\vspace{-15pt}
\small
\caption{\small \textbf{Training and testing at different crop scales.}}%
\begin{tabular}{@{}lrrrr@{}}
\toprule
Scale factor  & \multicolumn{1}{l}{PA-MPJPE} & \multicolumn{1}{l}{MPJPE} & \multicolumn{1}{l}{PA-PVE} & \multicolumn{1}{l}{PVE} \\ \midrule
Orig          & 9.56                         & 21.57                     & 9.26                       & 21.31                   \\
Tight crops & 8.73                         & 18.83                     & 8.52                       & 19.24                   \\ \bottomrule
\label{table:hand_scale}
\end{tabular}
\vspace{-15pt}
% \end{table}
\end{wraptable}

==> Tables/pw3d.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{0.50\textwidth}
% \begin{table}[]
\vspace{-35pt}
\small
\caption{\small \textbf{Evaluation of the Body sub-network}. We report PVE, MPJPE and PA-MPJPE.}%
\resizebox{.5\textwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Method}                     & PVE   & MPJPE & PA-MPJPE \\ \midrule
HMR (Res50) \cite{Kanazawa2017}      & -     & 130   & 76.7     \\
GraphCMR (Res50) \cite{Kolotouros2021}  & -     & -     & 70.2     \\
SPIN (Res50) \cite{Kolotouros2019}     & 116.4 & 96.9  & 59.2     \\
HMR-EFT (Res50) \cite{Joo2021} & -     & -     & 54.3     \\
ROMP (Res50)    & 105.6 & 89.3  & 53.5     \\
PARE (Res50) \cite{Kocabas2021}     & 99.7  & 82.9  & 52.3     \\
PARE (HR32) \cite{Kocabas2021}      & 97.9  & 82    & 50.9     \\
PyMAF (Res50)\cite{Zhang2022}            & 94.4  & 79.7  & 49       \\
PyMAF (HR48) \cite{Zhang2022}             & 91.3  & 78    & 47.1     \\
Baseline (Res50)         & -      & 85.2      & 52.4         \\
Ours (Res50)             & -      & 80.8      &  49.8        \\
Baseline (HR48)          & -     & 84.5      & 50.3         \\
Ours (HR48)              & -     & 80.1      & 48.5         \\ \bottomrule
\label{table:pw3d}
\end{tabular}}
\vspace{-35pt}
% \end{table}
\end{wraptable}

==> Tables/stirling.tex <==
% \begin{wraptable}{r}{0.40\textwidth}
% \begin{table}[]
\begin{wraptable}{r}{0.40\textwidth}
\vspace{-25pt}
\small
% \vspace{-10pt}
\centering
\caption{\small \textbf{Evaluation of the Face sub-network}. $\dagger$ denotes training with extra datasets.  }%
\vspace{-5pt}
\begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{@{}c|c|c|c@{}}
\begin{tabular}{@{}l|l@{}}
\Xhline{1pt}
\textbf{Model} & \textbf{Mean(mm) $\downarrow$} \\ \Xhline{1pt}
RingNet   &  2.08/2.02  \\
ExPose    &  2.27/2.42  \\
% Base        &  2.12/2.08  \\
ExPose $\dagger$        &  2.46/2.38  \\
\textbf{Ours}        &  \textbf{2.12/2.08}  \\
Ours $\dagger$        &  2.12/2.10  \\  \bottomrule
\end{tabular}

\end{adjustbox}
% \vspace{-10pt}
\label{table:stirling}
% \end{table}
\vspace{-15pt}
\end{wraptable}

==> Tables_Rebuttal/iou.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{wraptable}{l}{0.44\textwidth}
% \small
% \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}%
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{@{}llll@{}}
% \toprule
%            & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}}
% \end{wraptable}

% \begin{wrapfigure}{r}{0.44\textwidth} 
%     \centering
%     \subfigure{
%     \includegraphics[width=0.23\linewidth,keepaspectratio]{Figures_Rebuttal/Image/iou_calculation.png}
%     }
%     \caption{\small \textbf{Calculation for the Face, LHand and RHand IoU scores. The ground-truth and predicted part bounding boxes are denoted in green and red respectively.}}
%     \label{figure:vis}
% \end{wrapfigure}


% \begin{figure}
% \begin{floatrow}
% \ffigbox{%

%     \centering
%     \subfigure{
%     \includegraphics[width=0.5\linewidth,keepaspectratio]{Figures_Rebuttal/Image/iou_calculation.png}
%     }

% }{\caption{\small \textbf{Calculation for the Face, LHand and RHand IoU scores for ground-truth (green) and predicted (red) part bounding boxes.}}%
% }
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}llll@{}}
% \toprule
% Method     & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}%
% }
% \end{floatrow}
% \end{figure}

\begin{figure}
\begin{floatrow}
\ffigbox{%

    \centering
    \subfigure{
    \includegraphics[width=0.5\linewidth,keepaspectratio]{Figures_Rebuttal/Image/iou_calculation.png}
    }

}{\caption{\small \textbf{Calculation for the Face, LHand and RHand IoU scores for ground-truth (green) and predicted (red) part bounding boxes.}}%
}
\ffigbox{%

    \centering
    \subfigure{
    \includegraphics[width=0.5\linewidth,keepaspectratio]{Figures_Rebuttal/Image/pixel_alignment_quantitative.png}
    }
}{\caption{\small \textbf{Projected Vertex Errors is measured as distance between projected ground-truth (red) and predicted (blue) vertices in image space.}}%
}
\end{floatrow}
\end{figure}



==> Tables_Rebuttal/pixel_alignment.tex <==
% \begin{wraptable}{r}{0.44\textwidth}
% \small
% \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% Without Pixel Alignment Module                        & 11.796                                      \\
% With Pixel Alignment Module (vertex as supervision)   & 11.211                                      \\
% With Pixel Alignment Module (part seg as supervision) & 10.298                                      \\ \bottomrule
% \end{tabular}}
% \end{wraptable}

% \begin{wrapfigure}{r}{0.44\textwidth} 
% % \vspace{-20pt}
%     \centering
%     \subfigure{
%     \includegraphics[width=0.23\linewidth,keepaspectratio]{Figures_Rebuttal/Image/pixel_alignment_quantitative.png}
%     }
%     \caption{\small \textbf{We measure the distance between projected ground-truth and predicted vertices in image space denoted in red and blue respectively to obtain Projected Vertex Errors.}}
%     \label{figure:vis}
% % \vspace{-15pt}
% \end{wrapfigure}

% \begin{figure}
% \begin{floatrow}
% \ffigbox{%

%     \centering
%     \subfigure{
%     \includegraphics[width=0.5\linewidth,keepaspectratio]{Figures_Rebuttal/Image/pixel_alignment_quantitative.png}
%     }
% }{\caption{\small \textbf{We measure the distance between projected ground-truth and predicted vertices in image space denoted in red and blue respectively to obtain Projected Vertex Errors.}}%
% }
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% HMR                        & 11.796                                      \\
% HMR + PA (vertex)   & 11.211                                      \\
% HMR + PA (part-seg) & 10.298                                      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% }
% \end{floatrow}
% \end{figure}

% \begin{figure}
% \begin{floatrow}
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}llll@{}}
% \toprule
% Method     & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}%
% }
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% HMR                        & 11.796                                      \\
% HMR + PA (vertex)   & 11.211                                      \\
% HMR + PA (part-seg) & 10.298                                      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% }
% \end{floatrow}
% \end{figure}

% \begin{table}[t]
% \vspace{-5pt}
% \parbox{.45\linewidth}{
% \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}
% \small
% \resizebox{.45\textwidth}{!}{
% \begin{tabular}{@{}llll@{}}
% \toprule
% Method     & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}
% }
% }
% \hfill
% \parbox{.45\linewidth}{
% \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% \small
% \resizebox{.45\textwidth}{!}{
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% HMR                        & 11.796                                      \\
% HMR + PA (vertex)   & 11.211                                      \\
% HMR + PA (part-seg) & 10.298                                      \\ \bottomrule
% \end{tabular}

% }
% }
% \vspace{-20pt}
% \end{table}



% \begin{table}
% \parbox{.45\linewidth}{
% \small
% \centering
% \begin{tabular}{@{}llll@{}}
% \toprule
% Method     & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}
% \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}
% }
% \hfill
% \parbox{.45\linewidth}{
% \small
% \centering
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% HMR                        & 11.796                                      \\
% HMR + PA (vertex)   & 11.211                                      \\
% HMR + PA (part-seg) & 10.298                                      \\ \bottomrule
% \end{tabular}
% \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% }
% \end{table}


==> Tables_Rebuttal/pixel_alignment2.tex <==

% \begin{figure}
% \begin{floatrow}
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}llll@{}}
% \toprule
% Method     & Face IoU & LHand IoU & RHand IoU \\ \midrule
% ExPose     & 0.61     & 0.23      & 0.31      \\
% PIXIE      & 0.66     & 0.34      & 0.36      \\
% Hand4Whole & 0.75     & 0.41      & 0.45      \\
% OSX        & 0.70     & 0.38      & 0.41      \\
% RoboSMPLX  & 0.86     & 0.52      & 0.55      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}%
% }
% \capbtabbox{%

% \tiny
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% HMR                        & 11.796                                      \\
% HMR + PA (vertex)   & 11.211                                      \\
% HMR + PA (part-seg) & 10.298                                      \\ \bottomrule
% \end{tabular}
% }{%
%   \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% }
% \end{floatrow}
% \end{figure}


\begin{figure}
\begin{floatrow}
\capbtabbox{%

\tiny
\resizebox{.45\textwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
Method     & Face IoU \uparrow & LHand IoU \uparrow & RHand IoU \uparrow \\ \midrule
ExPose     & 0.61     & 0.23      & 0.31      \\
PIXIE      & 0.66     & 0.34      & 0.36      \\
Hand4Whole & 0.75     & 0.41      & 0.45      \\
OSX        & 0.70     & 0.38      & 0.41      \\
RoboSMPLX  & \textbf{0.86}     & \textbf{0.52}      & \textbf{0.55}      \\ \bottomrule
\end{tabular}}
}{%
  \caption{\small \textbf{Results for IoU of the predicted part bounding boxes on the EHF test set.}}%
}
\capbtabbox{%

\tiny
\resizebox{.42\textwidth}{!}{
\begin{tabular}{@{}ll@{}}
\toprule
Method                                                & \multicolumn{1}{c}{Projected Vertex Errors \downarrow } \\ \midrule
HMR (no PA)                       & 11.796                                      \\
HMR  + PA (vertex)   & 11.211                                      \\
HMR + PA (part-seg) & \textbf{10.298}                                      \\ \bottomrule
\end{tabular}
}}{%
  \caption{\small \textbf{Results of Projected Vertex Errors under different Part Alignment (PA)}}%
}
\end{floatrow}
\end{figure}

% \begin{wraptable}{r}{0.44\textwidth}
% \small
% \caption{\small \textbf{Results of Projected Vertex Errors under different training schemes.}}%
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{@{}ll@{}}
% \toprule
%                                                       & \multicolumn{1}{c}{Projected Vertex Errors} \\ \midrule
% Without Pixel Alignment Module                        & 11.796                                      \\
% With Pixel Alignment Module (vertex as supervision)   & 11.211                                      \\
% With Pixel Alignment Module (part seg as supervision) & 10.298                                      \\ \bottomrule
% \end{tabular}}
% \end{wraptable}
